Kauffman Skein Algebras and Quantum Teichm\"uller Spaces via Factorisation Homology

We compute the factorisation homology of the four-punctured sphere and punctured torus over the quantum group $\mathcal{U}_q(\mathfrak{sl}_2)$ explicitly as categories of equivariant modules using the framework of `Integrating Quantum Groups over Surfaces' by Ben-Zvi, Brochier, and Jordan. We identify the algebra of invariants (quantum global sections) with the spherical double affine Hecke algebra of type $(C^\vee_1,C_1)$, in the four-punctured sphere case, and with the `cyclic deformation' of $U(su_2)$ in the punctured torus case. In both cases, we give an identification with the corresponding quantum Teichm\"uller space as proposed by Teschner and Vartanov as a quantization of the moduli space of flat connections.

==> svg-macros.tex <==
% !TEX root=./main.tex
\makeatletter
\ifdefined\svgpath
% - Dynamically render images
\svgpath{{images/}{}}%
\newcommand{\myincludesvggroup}[4]{%
\renewcommand\svg@ink@area{}%
  \includesvg[#1,#2,inkscapename=#3-#4,inkscapeopt=-i\space#4\space-j]{#3}%
  \renewcommand\svg@ink@area{-C}%
}%
\else
% - Use prerendered images
% \newcommandx{\myincludesvg}[2][1=\linewidth,addprefix=\protected]{%
%     \def\svgwidth{#1}%
%     \import{svg-inkscape/}{#2_svg-tex.pdf_tex}%
% }%
% \newcommandx{\myincludesvgnolatex}[2][1=\linewidth,addprefix=\protected]{%
%     \includegraphics[width=#1]{svg-inkscape/#2_svg-raw.pdf}%
% }%
% /Users/julietcooke/Documents/SphericalDAHAs/
% /Users/julietcooke/Documents/SphericalDAHAs/
\newcommand{\svgroot}[0]{.}
\newcommand{\myincludesvg}[3]{\includegraphics[#1]{\svgroot/svg-inkscape/#3_svg-raw.pdf}}%
\newcommand{\myincludesvggroup}[4]{\includegraphics[#1]{\svgroot/svg-inkscape/#3-#4_svg-raw.pdf}}%
\fi
\makeatletter

%Test
% \svgpath{{/Users/julietcooke/Documents/SphericalDAHAs/images/}{}}
% \newcommand{\myincludesvg}[3]{\includesvg[#1,#2]{#3}}
% \makeatletter
% \newcommand{\myincludesvggroup}[4]{
% \renewcommand\svg@ink@area{}%
% \includesvg[#1,#2,inkscapename=#3-#4,inkscapeopt=-i #4 -j]{#3}%
% \renewcommand\svg@ink@area{-C}%
% }
% \makeatother

 %To load statically generated images
% \newcommand{\myincludesvg}[3]{\includegraphics[#1]{images_png/#3_svg-raw.png}}
% \newcommand{\myincludesvggroup}[4]{\includegraphics[#1]{images_png/#3-#4_svg-raw.png}}

\newcommand{\myincludesvgink}[3]{\myincludesvg{#1}{#2}{#3}}
\newcommand{\myincludesvggroupink}[4]{\myincludesvg{#1}{#2}{#3}{#4}}

\newcommand{\diagramhh}[5]{
\raisebox{-#3}{\myincludesvggroup{scale=#5}{inkscape=nolatex,inkscapeformat=pdf,inkscapename=#1-#2,inkscapeopt=-i #2 -j}{#1}{#2}}\hspace{#4}%
}
\newcommand{\diagramhhink}[5]{
\raisebox{-#3}{\myincludesvggroup{scale=#5}{inkscape=nolatex,inkscapeformat=pdf,inkscapename=#1-#2,inkscapeopt=-i #2 -j}{#1}{#2}}\hspace{#4}%
}
\newcommand{\smalldiagram}[2]{\diagramhh{#1}{#2}{18pt}{0pt}{0.75}}
\newcommand{\mediumdiagram}[2]{\diagramhh{#1}{#2}{20pt}{0pt}{0.75}}
\newcommand{\diagram}[2]{\diagramhh{#1}{#2}{23pt}{0pt}{0.75}}
\newcommand{\smallresult}[2]{\diagramhh{#1}{#2}{21pt}{0pt}{0.75}}
\newcommand{\skeindiagram}[1]{\diagramhh{skeinrelations}{#1}{10pt}{1pt}{0.25}}

